Attentive Fine-Grained Structured Sparsity for Image Restoration

Image restoration tasks have witnessed great performance improvement in recent years by developing large deep models. Despite the outstanding performance, the heavy computation demanded by the deep models has restricted the application of image restoration. To lift the restriction, it is required to reduce the size of the networks while maintaining accuracy. Recently, N:M structured pruning has appeared as one of the effective and practical pruning approaches for making the model efficient with the accuracy constraint. However, it fails to account for different computational complexities and performance requirements for different layers of an image restoration network. To further optimize the trade-off between the efficiency and the restoration accuracy, we propose a novel pruning method that determines the pruning ratio for N:M structured sparsity at each layer. Extensive experimental results on super-resolution and deblurring tasks demonstrate the efficacy of our method which outperforms previous pruning methods significantly. PyTorch implementation for the proposed methods is available at https://github.com/JungHunOh/SLS_CVPR2022.

==> Tables/Table4.tex <==
\begin{table}[t]
   \caption{Experimental results on the impact of the last layer in RFDN.
   The second row is the results of our method which is from Table~\ref{tab:sr_main_results}.
   From the searched pruning ratios in Figure~\ref{fig:searched_n:m}, we modify the layer-wise pruning ratios and prune the pre-trained RFDN network according to the modified ones.
   The re-training results of the pruned networks are shown in the last two rows.
   %`Searched by (method name)' means the layer-wise sparsity is searched by the proposed method and `Further pruned at the last layer' means the per-layer sparsity searched by (method name) is further increased at the last layer. We set $N$=4 at the last layer.
   }
   %\small
   \centering
   \scalebox{0.85}{
       \begin{threeparttable}
       \begin{tabular}{lccc}
           \toprule[\heavyrulewidth]
                  Layer-wise $N$:$M$ sparsity & GMACs & Num.Param. & PSNR$_\uparrow$\\
           \bottomrule[\heavyrulewidth]
           LS3 (Ours) & 5.16 & 139.60K & 25.58\\
           \midrule
           Set $N$=2 at the last layer & 4.46 & 127.50K & 25.39\\
           Fix the last layer and search & 4.46 & 122.13K & \textbf{25.47}\\
           \bottomrule[\heavyrulewidth]
       \end{tabular}
       \end{threeparttable}
   }
   \label{tab:exp_on_last_layer}
   %\vspace{0.1cm}
\end{table}

